G3DR: Generative 3D Reconstruction in ImageNet

We introduce a novel 3D generative method, Generative 3D Reconstruction (G3DR) in ImageNet, capable of generating diverse and high-quality 3D objects from single images, addressing the limitations of existing methods. At the heart of our framework is a novel depth regularization technique that enables the generation of scenes with high-geometric fidelity. G3DR also leverages a pretrained language-vision model, such as CLIP, to enable reconstruction in novel views and improve the visual realism of generations. Additionally, G3DR designs a simple but effective sampling procedure to further improve the quality of generations. G3DR offers diverse and efficient 3D asset generation based on class or text conditioning. Despite its simplicity, G3DR is able to beat state-of-theart methods, improving over them by up to 22% in perceptual metrics and 90% in geometry scores, while needing only half of the training time. Code is available at https://github.com/preddy5/G3DR

==> chapters/broader_impact.tex <==
\section*{Broader Impact}

G3DR and stronger models based on it can be used for a variety of applications, including:

\begin{itemize}
\item 3D modeling: G3DR can be used to generate 3D models of objects from single images. This can be useful for a variety of applications, such as product design, architectural visualization, and special effects.
\item Animation: G3DR can be used to generate 3D assets for animation, such as characters, props, and environments. This can help animators to create more realistic and visually appealing animations.
\item Video games: G3DR can be used to generate 3D assets for video games, such as characters, weapons, and vehicles. This can help game developers to create more immersive and engaging video games.
\end{itemize}


Unfortunately, G3DR, or more powerful models based on it can potential negative usages. One potential concern is that G3DR could be used to create realistic-looking fake images or videos (DeepFakes). This could be used for malicious purposes, such as spreading misinformation or propaganda.
%
In addition, G3DR could be used to create 3D models of people's faces or bodies without their consent. This could be used for privacy-violating purposes, such as tracking people or creating synthetic identities.
%
The authors do not endorse the usage of G3DR for any malicious purpose, such as deep fakes.



==> figures/ablation_geometry.tex <==
%\begin{table}[t!]
%\centering
%\begin{tabular}{lllll} 
%\toprule
%Method                            & 1       & 5        & 10       &50    \\ \hline
%Deng et al. 2022           & 26.96   &  27.85  & 26.21     & 22.4   \\ 
%WO Depth Regularization           & 32.58   &  24.91  & 22.34     & 19.38   \\ 
%Ours                              & 31.58   &  31.38  & 31.18     & 30.76  \\ 
%\bottomrule 
%\end{tabular}
%\caption{ablation geo}
%\label{res:ablation_geo}
%\end{table}

\begin{table*}[bth!]
\centering
\begin{tabular}{llllllllll} 
\toprule
  &  \multicolumn{3}{c}{Alternate Depth} & \multicolumn{3}{c}{} & \multicolumn{3}{c}{}\\
  &  \multicolumn{3}{c}{Supervision Loss} & \multicolumn{3}{c}{w/o Depth regularization} & \multicolumn{3}{c}{Ours}\\

Scaling factor  & FID $\downarrow$    & IS $\uparrow$    & NFS $\uparrow$ & FID $\downarrow$    & IS $\uparrow$    & NFS $\uparrow$ & FID $\downarrow$    & IS $\uparrow$    & NFS $\uparrow$         \\ \hline
1         &44.27  &83.04 & 28.96& 13.13 & 116.7& 36.58& 13.12 &151.72 & 36.51\\       
5         &128.64 &12.26 & 29.85& 73.34 & 26.72& 27.97& 12.98 &146.30 & 35.24\\       
10        &174.58 &5.33  & 26.21& 104.91& 14.07& 25.08& 14.42 &131.95 & 35.01\\       
50        &205.15 &3.58  & 22.42& 152.52& 5.94 & 19.38& 21.37 & 99.59 & 34.54\\       
\bottomrule 
\end{tabular}
\caption{Table quantifying the quality of geometry learned by models trained using different methods with various scaling factors.}
\label{res:ablation_geo}
\end{table*}

==> figures/grad_kernel_illustration_1d.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/images/1d_scaling.pdf}
    \caption{
    1d
    }
    \label{fig:illustration_1d}
    % \vspace{-10pt}
\end{figure}

==> figures/grad_kernel_illustration_2d.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/images/2d_scaling.pdf}
    \caption{
    2d
    }
    \label{fig:illustration_2d}
    % \vspace{-10pt}
\end{figure}

==> figures/rebuttal_fig.tex <==
\begin{figure*}[b]
    \centering
    \subfloat[Ablation VGG Loss and TV loss]{
        \begin{tabular}{lllll} 
\toprule
Method                            & FID $\downarrow$    & IS $\uparrow$    & NFS $\uparrow$ \\  \hline
w/o VGG Loss           &  18.4 & 126.5&  36.4     \\ 
%WO Percep                  & 42.71  & 47.93 & 35.92 \\
w/o TV loss                  & 15.0  & 139.2 & 35.8 \\ \hline
Ours                              & \textbf{13.1}    &  \textbf{151.7}     & \textbf{36.5}   \\ 
\bottomrule 
    \label{tab:ablation_vgg_tv}
\end{tabular}
%\caption{The effect of each block in our framework. }

    }
    \subfloat[Clip Embeddings Cosine Similarity]{           
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/images/clip_image_2_2.png}
    %\caption{
    %Scatter plot of Cosine Similarity between random views of the same scene vs other scenes. The images on the bottom show the canonical view of the generated scenes. The plots in green contain a mean value $>$0.92 and the plots in red contain a mean value $<$0.58.
    %}
    \label{fig:clip_image}

}
    \subfloat[Qualitative Comparison]{           
    \centering
    \includegraphics[width=0.65\columnwidth]{figures/images/qualitative_3_crop.png}
    %\caption{
    %Scatter plot of Cosine Similarity between random views of the same scene vs other scenes. The images on the bottom show the canonical view of the generated scenes. The plots in green contain a mean value $>$0.92 and the plots in red contain a mean value $<$0.58.
    %}
    \label{fig:qualitative2}
}
    %\caption{
    %Tab.~\ref{tab:ablation_vgg_tv} We ablated the effect of VGG loss and TV loss on generation quality. Fig.~\ref{fig:clip_image} Scatter plot of Cosine Similarity between random views of the same scene vs other scenes. The images on the bottom show the canonical view of the generated scenes. The plots in green contain a mean value $>$0.92 and the plots in red contain a mean value $<$0.58. Fig.~\ref{fig:qualitative2} A 2-row sample of the proposed qualitative comparison visualization we will add to the final paper. \textit{Please use digital zoom to view the images more clearly}.
    %}
\end{figure*}

==> figures/scaling_factor.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/images/scale_factor.pdf}
    \caption{Visualization of $f_{trigen}$ outputs rendered using different scale factors. Notice how the results generated by the model trained using our method degrade gracefully.
    }
    \label{fig:scaling_factor}
    % \vspace{-10pt}
\end{figure}

==> tables/recon_metric.tex <==
\begin{table}[ht]
\centering
\resizebox{0.32\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
& FID $\downarrow$    & IS $\uparrow$ & NFS $\uparrow$  & DA $\uparrow$ \\ \hline
Ours& \textbf{11.25}    &  \textbf{168.6}&  \textbf{36.7} &  \textbf{0.33}    \\ 
\bottomrule 
\end{tabular}}
\caption{Quantitative evaluation of novel view generation using images from ImageNet dataset.}
\label{res:recon_metric}
\end{table}
